Synthesizing Multimodal Electronic Health Records via Predictive Diffusion Models

Synthesizing electronic health records (EHR) data has become a preferred strategy to address data scarcity, improve data quality, and model fairness in healthcare. However, existing approaches for EHR data generation predominantly rely on state-of-the-art generative techniques like generative adversarial networks, variational autoencoders, and language models. These methods typically replicate input visits, resulting in inadequate modeling of temporal dependencies between visits and overlooking the generation of time information, a crucial element in EHR data. Moreover, their ability to learn visit representations is limited due to simple linear mapping functions, thus compromising generation quality. To address these limitations, we propose a novel EHR data generation model called EHRPD. It is a diffusion-based model designed to predict the next visit based on the current one while also incorporating time interval estimation. To enhance generation quality and diversity, we introduce a novel time-aware visit embedding module and a pioneering predictive denoising diffusion probabilistic model (PDDPM). Additionally, we devise a predictive U-Net (PU-Net) to optimize P-DDPM.We conduct experiments on two public datasets and evaluate EHRPD from fidelity, privacy, and utility perspectives. The experimental results demonstrate the efficacy and utility of the proposed EHRPD in addressing the aforementioned limitations and advancing EHR data generation.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> files/1-intro.tex <==
\section{Introduction}

\begin{figure}[]
    \centering
\includegraphics[width=0.85\columnwidth]{figure/piplineplot.pdf}
    \vspace{-2mm}
    \caption{Pipeline of existing methods vs. {\ours}.}
    \label{pipeline}
\end{figure}

In the rapidly evolving landscape of healthcare, using Electronic Health Records (EHR) data is central to advancing data-driven methods in both research and clinical practice~\cite{xiao2018opportunities}. EHR data, comparing patients' time-ordered sequences of clinical visits, encapsulate crucial information for patient care. However, effectively leveraging this complex data form faces a significant challenge due to the scarcity of high-quality EHR datasets. To overcome this challenge, EHR data generation become a vital solution, offering a way to create synthetic yet realistic supplements of patient data for building robust healthcare application models.

Recent advancements in EHR data generation adopt Generative Adversarial Networks (GAN)~\cite{medGAN,ehrGAN,synteg}, Variational Autoencoders (VAE)~\cite{twin,eva}, and Language Models (LM)~\cite{promptehr,HALO} as generators. Their generation pipeline can be simplified and visualized in Figure~\ref{pipeline}. A raw, multi-hot encoded visit $V_i$ is first fed through an encoder $E$ to produce dense visit embedding $\mathbf{v}_i$. Then a generating module $M$ produces a synthetic $\hat{\mathbf{v}}_i$ from $\mathbf{v}_i$, and a decoder map it to the original data space. However, the existing EHR data generation methods generally face the following drawbacks:

\begin{itemize}
    \item \textbf{(1):} Existing methods are built in a visit-replicating style,i.e., generating $\hat{V}_i$ from $V_i$. However, this generation style inherently downplay the complex temporality of EHR data.
    \item \textbf{(2):} Existing methods generally utilize a linear layer to produce code embedding. This simple method might not able to model the nuance code-level temporality.
    \item \textbf{(3):} Existing GAN-based method faces model collapsing issue during training. VAE-based method is constrained by its Gaussian assumption of latent space that does generalize well if data is non
\end{itemize}






% In the rapidly evolving landscape of healthcare, the utilization of Electronic Health Records (EHR) data is central to the advancement of data-driven methodologies in both research and clinical practice~\cite{xiao2018opportunities}. EHR data, comprising patients' time-ordered sequences of clinical visits, encapsulate crucial information for patient care. However, effectively leveraging this complex data form presents a significant challenge due to the scarcity of high-quality EHR datasets, often caused by limited access to patient data and privacy concerns. To overcome this challenge, EHR data generation emerges as a pivotal solution, offering a way to create synthetic yet realistic supplements of patient data for building robust healthcare application models. 

Recent advancements leverage generative networks to combat the data scarcity challenge. Generative Adversarial Network (GAN)~\cite{medGAN,ehrGAN,synteg}, Variational Autoencoder (VAE)~\cite{twin,eva}, and Language Model (LM)~\cite{promptehr,HALO} are among the most researched techniques that foster the applications of EHR generation methods. 
% On the other hand, the Denoising Diffusion Probabilistic Model (DDPM) has seen great success in other domains, such as image generation~\cite{glide}, time-series forecasting~\cite{rasul2021autoregressive}, and text generation~\cite{gong2022diffuseq}. Recent work also introduces DDPM to the medical field, generating tabular healthcare data~\cite{tabddpm} or performing task-specific data agumentation~\cite{meddiffusion}. Their development marks a crucial step in leveraging deep learning methods to fill research gaps in EHR data generation. 
However, existing EHR generation techniques still face the following drawbacks:
\begin{itemize}
    % \item \textbf{(1) Reliance on fixed-size training data:} A common drawback of existing EHR generation models based on GANs, VAEs, and LMs is their direct dependency on the data available for training. In a self-supervised manner, these models are trained or fine-tuned on a fixed and relatively small training set. This limits the performance of the generation models as well as the diversity of generated outputs. In contrast, the DDPM introduces a unique method of implicit data augmentation. By adding varying levels of noise to the input data during the forward diffusion process, DDPM effectively expands the training dataset, which not only combats the data scarcity issue but also helps the model to be robust against unrelated information. Thus the DDPM is particularly advantageous in the health domain where data is scarce. 

    % \item \textbf{(1) Model specific weaknesses:} Given the multimodal and high-dimensional characteristics of EHR data, evaluating the strengths and weaknesses of generative models considering the limited data availability becomes essential. GAN-based approaches\cite{xu2019modeling} often struggle to model the complex relationships among high-dimensional codes across different modalities and also frequently face the model collapsing issue. In contrast, VAEs, constrained by their Gaussian distribution assumption of the latent space~\cite{xu2019modeling}, fail to fully capture the data's diversity and complexity. Although potent in their capability, LMs that are trained on large, general corpora can inadvertently introduce irrelevant information into domain-specific tasks. DDPMs, however, stand out by offering a stable training experience and a balance between model complexity and the limitations imposed by data scarcity. This balance positions DDPMs as particularly well-suited for the task of generating synthetic EHR data in healthcare, outweighing other generative models in terms of both feasibility and effectiveness.

    \item \textbf{(1) Unable to model the complex code relation effectively:}
    Existing EHR generation models that are based on VAE, GAN, and LM struggle with accurately modeling the intricate relationships and dependencies in the EHR data. GAN-based models~\cite{medGAN,ehrGAN,synteg} discard nuance information by either aggregating variables to the patient level or largely reducing the code vocabulary size. VAE-based models~\cite{eva,twin} aim to generate low-dimensional EHR or trial data, limiting its ability to be applied to a complex setting. LM-based methods~\cite{promptehr,HALO}, when not fine-tuned with sufficient EHR data, can introduce irrelevant or inaccurate information which harms the generation performance. In contrast, the iterative process of noise addition and deletion enables the diffusion model to accurately capture the complex EHR data distribution while keeping the diversified nature of the generated data.
    
    \item \textbf{(2) Neglect of Modeling and Producing Temporal Information:} Existing models designed to produce fine-grain data often miss a key aspect of patient healthcare: the time information. Risk prediction models~\cite{hitanet,lsan} utilize time information as a crucial feature to model the disease progression. However, existing generation models cannot produce synthetic data with such information and this oversight hinders the performance of time-based predictive models on synthetic data. Therefore, despite the progress made, there is a need for models that can generate detailed and accurate patient data and provide the critical time dimension of patient health trajectory.
\end{itemize}

To address those drawbacks, a naive solution is to utilize DDPM in a same-visit generation approach as well as modeling time information like~\cite{meddiffusion}. However, the sequential characteristics of EHR data pose a serious challenge that needs to be addressed: the same-visit generation DDPM is found lacking in preserving the sequential information in a fine-grained visit-level manner.

\begin{figure}[]
    \centering
\includegraphics[width=0.85\columnwidth]{figure/codetimeplot.pdf}
    \vspace{-2mm}
    \caption{Illistration of multimodal EHR data with the code-level time gap.}
    \label{codetime}
\end{figure}



% However, it is found lacking due to its visit-replicating generation style. In contrast, a visit-to-next-visit approach can naturally capture the evolution of a patient's condition, learning to a better quality of generated data. However, this method requires careful modification to the existing DDPM architecture.

% \textbf{Same-visit replicating generation style:} Existing works of EHR generation with DDPM primarily focus on a same-visit generation approach that is designed to replicate and perturb the patient data. This method can be beneficial in capturing the general characteristics of the patient's records but inherently lacks the capability of modeling the disease progression sequentially since it neither explicitly predicts future situations nor models the transition between visits. In contrast, a visit-to-next-visit approach can naturally capture the evolution of a patient's condition, learning to a better quality of generated data. However, this method requires careful modification to the existing DDPM architecture.

To address the above issue, we propose \ours, a visit-to-next-visit diffusion model that also provides synthetic time for EHR data generation. It consists of three main components: the Predictive Denoising Diffusion Probabilistic
Models (\dmodel), the time-aware visit embedding, and catalyst representation learning. The \dmodel aims to generate the next visit with a special \unet, conditional on catalyst representation. The Time-aware visit embedding module models the fine-grained code-time relationship and produces visit embedding for \unet. The catalyst representation learning module produces predicted time gap, demographic information, and medical history as generation conditions of \unet. Figure~\ref{mainModel} shows the structure of \ours.

\begin{figure*}[]
    \centering
\includegraphics[width=0.85\textwidth]{figure/mainplot.pdf}
    \vspace{-2mm}
    \caption{Overview of the proposed {\ours} model.}
    \label{mainModel}
\end{figure*}

To sum up, our contributions are listed as follows: (1) To the best of our knowledge, this is the first work to generate EHR codes and time gaps with the diffusion model in a visit-to-next-visit manner. (2) We propose \ours that not only considers the hidden relationship between code and time but also provides explicit time predictions as output. (3) We conduct extensive experiments from different aspects on public MIMIC-III and Breast Cancer Trial databases to demonstrate the effectiveness of our model.



% Some existing work~\cite{medGAN,tabddpm} generates patient-level data that leverage Generative Adversarial Network (GAN)~\cite{gan} or Denoising Diffusion Probablisitc Model (DDPM)~\cite{ddpm}, which is instrumental in offering an overview of patient medical condition across broader healthcare contexts. Others~\cite{promptehr,synteg,twin,eva,HALO} aim to provide more detailed, fine-grained admission-level synthetic EHR data. Their development marks a crucial step in leveraging deep learning methods to fill research gaps in EHR data generation.

% In the rapidly evolving landscape of healthcare, the utilization of Electronic Health Records (EHR) data is central to the advancement of data-driven methodologies in both research and clinical practice~\cite{xiao2018opportunities}. EHR data, comprising patients' time-ordered sequences of clinical visits, encapsulate crucial information for patient care. Each visit is detailed with high-dimensional yet discrete medical codes, such as the International Classification of Disease (ICD) codes, giving a comprehensive picture of a patient's health history. However, effectively leveraging this rich, complex data presents a significant challenge due to the scarcity of high-quality EHR datasets. This scarcity is often compounded by issues such as limited access to patient data, privacy concerns, and inconsistencies in data collection across healthcare settings. To overcome these challenges, the generation of EHR data emerges as a pivotal solution, offering a way to create synthetic yet realistic supplements of patient data. Such generated data not only aids in tailored treatments and risk predictions for enhanced patient analysis but also can contribute to the broader context of healthcare research and practice. To this end, it is critical to develop methods of generating synthetic data that accurately and comprehensively reflect the complex and dynamic nature of real EHR data.



% Recent advancements in EHR data generation have primarily focused on addressing the challenge of data scarcity in both fine-grain and course-grain scopes. Some existing work~\cite{medGAN,tabddpm} generates patient-level data that leverage Generative Adversarial Network (GAN)~\cite{gan} or Denoising Diffusion Probablisitc Model (DDPM)~\cite{ddpm}, which is instrumental in offering an overview of patient medical condition across broader healthcare contexts. Others~\cite{promptehr,synteg,twin,eva,HALO} aim to provide more detailed, fine-grained admission-level synthetic EHR data. Their development marks a crucial step in leveraging deep learning methods to fill research gaps in EHR data generation. Despite these advancements, existing models in EHR data generation reveal notable shortcomings that limit their effectiveness in practical healthcare applications:

% \begin{itemize}

%     % \item \textbf{Lack of Details by Patient-level Generation:} While models for generating patient-level data help mitigate the issue of data scarcity, they frequently fall short in accurately replicating the detailed and coherent medical histories essential for comprehensive analysis. This shortcoming is often due to the inherent limitations in their design, which provide a summarization of the patient's history, instead of the nuanced, individualized details critical for a truly fine-grained and realistic representation.
%     \item \textbf{Neglect of Modeling and Producing Temporal Information:} Additionally, even the models designed to produce more granular data often miss a key aspect of patient healthcare: the temporal dynamics. Important factors such as the intervals between hospital admissions and the progression of diseases over time are frequently neglected. This oversight results in a gap in these models' ability to simulate patient health trajectories realistically. Therefore, despite the progress made, there exists a need for models that can not only generate detailed and accurate patient data but also incorporate the critical temporal dimensions of patient health.
% \end{itemize}

% To address these shortcomings in current EHR data generation models, we propose \ours. Our model is designed to target the details of EHR codes and accurately model the temporal progression of patient health conditions. Section~\ref{main} describes the foundations of our step-wise approach to generate synthetic visits with a diffusion model. Section~\ref{unet} presents our Step-wise Visit Generation Module to handle the generation process. Section~\ref{visitemb} shows our fine-grained approach to modeling the code-time relationship and constructing visit embedding. Section~\ref{conditionalemb} discusses how we construct the conditional information matrix as extra input for the generation module.





==> files/3-model-old.tex <==
\section{Model Architecture}

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.9\textwidth]{figure/model.jpg}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure*}


\subsection{Overview}

Our model is designed to analyze healthcare data in a step-by-step manner. It starts by converting the data into a dense format. Next, it examines the appearance and timing of each medical code to model codes temporally. The model then summarizes these codes into visit-level and estimates the time until the next healthcare visit, mimicking a doctor planning follow-up appointments. To predict future visits, it uses a diffusion model that gradually builds up each visit's details conditional on previous medical history, current conditions, and the predicted time gap. Lastly, an MLP is used to predict the codes of the next visit from the reconstructed results.




\subsection{Problem Formulation and Data Representation}

There are a total of $N$ patients in each of the selected databases. The $n$-th patient's medical history is a sequence of visits indexed by $i$, and can be represented in temporal order as:

\begin{equation}
    X_{n}^{1:I} = \{x_n^1, x_n^2, \cdots, x_n^I\},
\end{equation}
where $I$ is the last visit of the patient and can be different for each patient. For the sake of readability, we treat $x^i$ as $x^i_n$ in the following discussion. This representation encompasses all modalities associated with the visit, and we can represent a patient's medical record by modalities at $i$-th visit as:

\begin{equation}
    x^i = \{x^i_1, x^i_2, \cdots, x^i_U\},
\end{equation}
where $U$ is the total number of modalities in the data. Then $x^i_u$ contains a set of codes of modality $u$ from $i$-th visit of the patient and can be denoted as $x^i_u = \{c^i_{u,1}, c^i_{u,2}, \cdots, c^i_{u,M}\}$, where $M$ is the total number of codes. $c^i_{u,m} \in \{0,1\}$ is a binary indicator of the presence of the code.

% Besides the medical codes, we also include the time interval between the $i$-th visit and the $i+1$-th visit in our study, denoted as $\Delta t^i$. Furthermore, we calculate and construct a fine-grained code-level time interval for each modality. The time interval of the first appearance of the $m$-th code of modality $u$ is set to $0$. Then the following time interval is the difference between the current appearance of the same code against its last appearance. 

Besides the medical codes, we track the time gap between each patient's visits. We label the time between the $i$-th and $i+1$-th visit as $\Delta t^i$. We also look closely at the time intervals for each individual medical code. When the $m$-th code of modality $u$ shows up for the first time, we mark its time interval $\Delta t^1_{u,m}$ as $0$. For any later appearances of this same code, we calculate the time interval $\Delta t^i_{u,m}$ as the difference in time between this new appearance and when it last appeared. These time gap calculations are integral to our analysis, enabling a nuanced understanding of patient care patterns across different modalities, which will be further explored in subsequent sections.

\subsection{Code-time Information Modeling}
For modality presented in a patient's $i$-th diagnosis, an embedding layer can be used to transform its discrete codes into dense embedding $\mathbf{c}_m$ of dimension $d$. Then the visit level embedding $\mathbf{v}^i$ can be obtained by taking the summation of code embedding within $i$-th visit. However, the embedding $\mathbf{v}^i$ is static and doesn't encapsulate the temporal evolution of the disease across multiple visits. To address this deficiency, our approach aims to capture the temporal dynamics of each medical code individually by modeling with the code-level time gap vectors and is detailed in this section.

\subsubsection{Fine-grained Code-time Embedding:}
For code $c^i_{u,m}$ in modality $u$ and its respective code level time gap vector $\Delta t^i_{u,m}$, an embedding layer transforms the discrete code into a dense embedding $\mathbf{c}^i_{u,m}$  of dimension $d$. The code embedding is then merged with the corresponding time gap embedding \( \Delta t^i_{u,m} \), forming $\mathbf{\eta}^i_{u,m}$ by the same equation across all modalities as follows:

\begin{equation}
\begin{gathered}
    \mathbf{\eta}^i_{u,m} = f(\mathbf{c}^i_{u,m}, \mathbf{\Delta t}^i_{u,m}) g(\mathbf{c}^i_{u,m}, \mathbf{\Delta t}^i_{u,m}) + (1- f(\mathbf{c}^i_{u,m}, \mathbf{\Delta t}^i_{u,m}) \mathbf{c}^i_{u,m}.
\end{gathered}
\label{eq:timeEncoding}
\end{equation}

In the above Eq.~\ref{eq:timeEncoding}, we utilize the positional encoding method with feed-forward layers to encode the code level time gap $\Delta t^i_{u,m}$ into dense embedding $\mathbf{\Delta t}^i_{u,m}$ of dimension $d$, as follows:

\begin{equation}
\begin{gathered}
\mathbf{\Delta t}^i_{u,m} = \mathbf{W}_{t_2} \left(\sigma\left(\mathbf{W}_{t_1} \text{PE}(\Delta t^i_{u,m}) + \mathbf{b}_{t_1}\right)\right) + \mathbf{b}_{t_2},\\
\text{PE}(\Delta t^i_{u,m}, 2k) = \sin\left(\frac{\Delta t^i_{u,m}}{10000^{\frac{2k}{d}}}\right),\\
\text{PE}(\Delta t^i_{u,m}, 2k+1) = \cos\left(\frac{\Delta t^i_{u,m}}{10000^{\frac{2k}{d}}}\right),
\end{gathered}
\end{equation}
where $k = [0, 1, \cdots, \frac{d}{2}-1]$, $\mathbf{W}_{t_1}, \mathbf{W}_{t_2} \in \mathbb{R}^{d*d}$, and $\mathbf{b}_{t_1}, \mathbf{b}_{t_2} \in \mathbb{R}^d$.

The function $f(\mathbf{c}^i_{u,m}, \mathbf{\Delta t}^i_{u,m})$ in Eq.\ref{eq:timeEncoding} produces a binary output that represents whether the presented code embedding $\mathbf{c}^i_{u,m}$ should be modified based on the time gap information $\mathbf{\Delta t}^i_{u,m}$. We employ a Gumbel-Softmax layer to sample from this decision-making process while keeping it differentiable as follows:

\begin{equation}
    \begin{aligned}
        f(\mathbf{c}^i_{u,m}, \mathbf{\Delta t}^i_{u,m}) &= \text{Binarize}\left( \frac{\exp\left(\frac{\log(\mathbf{p}^i_{u,m}[0]) + g_0}{\tau}\right)}{\sum_{j=0}^{1} \exp\left(\frac{\log(\mathbf{p}^i_{u,m}[j]) + g_j}{\tau}\right)} \right), \\
        \mathbf{p}^i_{u,m} &= \text{Softmax}(\mathbf{W}_p [\mathbf{c}^i_{u,m}, \mathbf{W}_t \mathbf{\Delta t}^i_{u,m}] + \mathbf{b}_p).
    \end{aligned}
\label{eq:gumbel}
\end{equation}

The above code-time embedding process mimics how a healthcare professional monitors a patient's health. By observing the timing and frequency of each code, the model identifies patterns and trends in each disease progression. This temporal analysis helps the model to determine when to update its information, leading to more precise and timely predictions about disease progression.

\subsubsection{Aggregated Visit-level Embedding:}
To dynamically acquire the most relevant information from each modality, we utilize a modality-level attention layer to dynamically aggregate embedding, which is defined as follows:

\begin{equation}
    \mathbf{s}^i_{u} = \sum_{m=1}^{M_{u}} \mathbf{\eta}^i_{u,m},
\end{equation}
where \( M_{u} \) denotes the number of codes in modality $u$. The aggregated vector for each modality is transformed via a feed-forward layer:

\begin{equation}
    \mathbf{z}^i_{u} = \text{ReLU}(\mathbf{W}_{u} \mathbf{s}^i_{u} + \mathbf{b}_{u}),
\end{equation}
where $\mathbf{W}_{u}\in \mathbb{R}^{d*d}, \mathbf{d}_{u} \in \mathbb{R}^d$. The attention scores for the modalities are computed collectively as:

\begin{equation}
    \mathbf{a}^i = \text{Softmax}(\mathbf{W}_{a} [\mathbf{z}^i_{1}, \mathbf{z}^i_{2},\cdots, \mathbf{z}^i_{U}] + \mathbf{b}_{a}),
\end{equation}
where $\mathbf{W}_{a}\in \mathbb{R}^{4*d} $ and $ \mathbf{d}_{a} \in \mathbb{R}^{d}$. The final visit-level embedding is computed by the weighted sum of embeddings:

\begin{equation}
    \mathbf{v}^i = \sum_{u=1}^{U} a^i_{u} \mathbf{z}^i_{u},
\end{equation}
where  $\mathbf{v}^i \in \mathbb{R}^d$ .

\subsubsection{Demographic Information:}

We also incorporate demographic information for each patient as a multi-hot encoded vector \(\mathbf{D}\) and embed it into the same dense dimension $d$ using a linear layer:

\begin{equation}
    \mathbf{De} = \mathbf{W}_D\mathbf{D} + \mathbf{b}_D,
\end{equation}
where $\mathbf{W}_D \in \mathbb{R}^{d*d}$ and $ \mathbf{b}_D \in \mathbb{R}^d$ .

\subsection{Hidden State Learning and Time Gap Prediction}

In the development of our model, we draw inspiration from the decision-making methodologies employed by healthcare practitioners. Analogous to how a clinician considers both past medical records and present health indicators to settle down the appropriate interval till the follow-up visit, we process historical medical data in conjunction with current medical codes to forecast the ideal timing for subsequent visits. Following the work of continuous-time LSTM with Hawkes Process~\cite{hawkeslstm}, we first generate a current visit hidden state based on the learned visit embedding, as follows:

\begin{equation}
    \mathbf{h}^i = \text{LSTM}(\mathbf{h}^{i-1},\mathbf{v}^i).
\end{equation}
We then employ a two-step linear transformation to predict the time gap, as shown in Eq.\ref{eq:timepred}. We first utilize a linear layer on hidden state $\mathbf{h}^i$ to learn an intensity measure $\lambda^i(t)$ of the current visit, which represents a patient's medical urgency. This intensity is subtracted from $1$, giving a close to $0$ output if the patient's condition is urgent. Then the second equation predicts the time gap and ensures it is strictly above $0$ with the Softplus activation function:

\begin{equation}
\begin{aligned}
    \mathbf{\lambda^i(t)} &= 1 - \text{tanh}(\mathbf{W}_\lambda \mathbf{h}^i + \mathbf{b}_\lambda),\\
    \Delta \hat{t}^i &= \text{Softplus}(\mathbf{W}_{\hat{t}} \mathbf{\lambda^i(t)} + \mathbf{b}_{\hat{t}}).
\end{aligned}
\label{eq:timepred}
\end{equation}
where $\mathbf{W}_\lambda \in \mathbb{R}^{d\times d}; \mathbf{W}_{\hat{t}}, \mathbf{b}_{\lambda},$ and $ \mathbf{b}_{\hat{t}} \in \mathbb{R}^{d}$.

\subsection{Generation of Next Visit}

\subsubsection{Forward Diffusion Process}

Different from the existing work that aims to reconstruct synthetic $i$-th visit by a noised $i$-th visit, our modified diffusion process seeks to predict the $i+1$-th visit instead, conditional on various information. Let $\tau$ denote the diffusion time step, and $\beta_\tau$ denote the variance schedule of $\tau$. We treat the concatenation of all modalities as one during the diffusion process: $\mathbf{\eta}^i = [\mathbf{\eta}^i_{1},\mathbf{\eta}^i_{2},\cdots,\mathbf{\eta}^i_{U}]$. In mathematical terms, our forward diffusion process can be written in the following way:

\begin{equation}
\begin{gathered}
    q(\mathbf{\eta}^i_{1:T}|\mathbf{\eta}^i_0)=\prod^T_{\tau=1}q(\mathbf{\eta}^i_{\tau-1}),\\
    q(\mathbf{\eta}^i_{\tau}|\mathbf{\eta}^i_{\tau-1}) = \mathcal{N}(\mathbf{\eta}^i_\tau;\sqrt{1-\beta_\tau}\eta^i_{\tau-1},\beta_\tau \mathbf{I}).
\end{gathered}
\end{equation}

With $\alpha_\tau = 1-\beta_\tau$ and $\tilde{\alpha}_\tau = \prod^T_{j=1}\alpha_j$, we can reparameterize $\mathbf{\eta}^{i}_{\tau}$ and $\mathbf{\eta}^{i+1}_{\tau}$ as follows:

\begin{equation}
\begin{gathered}
    \mathbf{\eta}^{i}_{\tau} = \sqrt{\alpha_\tau} \mathbf{\eta}^{i}_{\tau-1} + \sqrt{1-\alpha_\tau}\epsilon_{t-1} 
    = \sqrt{\tilde{\alpha}_\tau} \mathbf{\eta}^{i}_{0} + \sqrt{1-\tilde{\alpha}_\tau}\epsilon,\\
    \mathbf{\eta}^{i+1}_{\tau} = \sqrt{\alpha_\tau} \mathbf{\eta}^{i+1}_{\tau-1} + \sqrt{1-\alpha_\tau}\epsilon_{t-1}
    = \sqrt{\tilde{\alpha}_\tau} \mathbf{\eta}^{i+1}_{0} + \sqrt{1-\tilde{\alpha}_\tau}\epsilon,
\end{gathered}
\end{equation}

\subsubsection{Assumption}

Although $\mathbf{\eta}^{i}_{0}$ and $\mathbf{\eta}^{i+1}_{0}$ are distinctive visit samples, they are close in the sample space since they are consecutive and are from the same patient. And during the forward diffusion process, $\eta^{i}_{\tau}$ and $\eta^{i+1}_{\tau}$ become more and more indistinguishable with the corruption of noise $\epsilon_\tau$, and as $T \to \infty$, $\eta^{i}_{T}$ and $\eta^{i+1}_{T}$ lie in the same Gaussian distribution of $\mathcal{N}(0,\mathbf{I})$. Thus we make the following assumption that during the noise addition trajectory, the noised $i+1$-th code embedding matrix can be considered as the summation of the $i$-th code embedding matrix and extra information $o(\mathbf{H}^{i}_{\tau})$: $\phi^i \mathbf{\eta}^{i}_{\tau}+ (1-\phi^i) o(\mathbf{H}^{i}_{\tau}) = \mathbf{\eta}^{i+1}_{\tau}$, where $\tau \in (1, T)$ and $o(\mathbf{H}^{i}_{\tau}) = o(\mathbf{\mathbf{h}^i, \Delta\mathbf{\hat{t}}}^{i}_{\tau}, \mathbf{De}, \mathbf{U})$, and $\phi^i$ is a weighting vector. This allows us to first use the forward diffusion process on $\mathbf{\eta}^{i}_{0}$ and $o(\mathbf{H}^{i}_{0})$ to obtain $\mathbf{\eta}^{i+1}_{T} = \mathbf{\eta}^{i}_{T} + o(\mathbf{H}^{i}_{T})$, and then denoise from $\mathbf{\eta}^{i+1}_{T}$ to construct code embedding at $i+1$-th visit $\hat{\mathbf{\eta}}^{i+1}_{0}$, without the real $\mathbf{\eta}_0^{i+1}$.

Thus we can write $\mathbf{\eta}^{i+1}_{\tau}$ as:

\begin{equation}
    \begin{gathered}
        \mathbf{\eta}^{i+1}_{\tau} = \phi^i \mathbf{\eta}^{i}_{\tau} + (1-\phi^i) o(\mathbf{H}^{i}_{\tau}) \\ = \sqrt{\tilde{\alpha}_\tau}(\phi^i \mathbf{\eta}^{i}_{0} + (1-\phi^i) o(\mathbf{H}^{i}_{0})) + 2\sqrt{1-\tilde{\alpha}_\tau}\epsilon_\tau, \\
        \frac{1}{\sqrt{\tilde{\alpha}_\tau}}(\mathbf{\eta}^{i+1}_{\tau} - 2\sqrt{1-\tilde{\alpha}_\tau}\epsilon_\tau) = \phi^i \mathbf{\eta}^{i}_{0} + (1-\phi^i) o(\mathbf{H}^{i}_{0}).
    \end{gathered}
\label{eta_rewrite}
\end{equation}

\subsubsection{Backward Diffusion Process}

Starting to denoise the $\mathbf{\eta}^{i+1}_{\tau}$, the backward diffusion steps can be written by the Bayes Theorem as follows:

\begin{equation}
    \begin{gathered}
        q(\mathbf{\eta}^{i+1}_{\tau-1}|\mathbf{\eta}^{i+1}_{\tau},\mathbf{\eta}^{i+1}_{0}) = q(\mathbf{\eta}^{i+1}_{\tau}|\mathbf{\eta}^{i+1}_{\tau-1},\mathbf{\eta}^{i+1}_{0}) \frac{q(\mathbf{\eta}^{i+1}_{\tau-1}|\mathbf{\eta}^{i+1}_{0})}{q(\mathbf{\eta}^{i+1}_{\tau}|\mathbf{\eta}^{i+1}_{0})},
    \end{gathered}
\end{equation}
Then we can obtain the mean $\tilde{\beta}_\tau$ and variance $\tilde{\mu}_\tau(\mathbf{\eta}^{i+1}_\tau, \mathbf{\eta}^{i+1}_0)$ of the backward process's cumulative distribution by the definition of normal distribution and some algebra, in terms of $\mathbf{\eta}^i_\tau$: 

% and by the definition of normal distribution, the cumulative distribution of the above equation is proportional to:

% \begin{equation}
%     \begin{gathered}
%         \propto exp \{ -\frac{1}{2} (\frac{(\eta^{i+1}_\tau-\sqrt{\alpha_\tau}\eta^{i+1}_{\tau-1})^2}{\beta_\tau} 
%         + \frac{(\eta^{i+1}_{\tau-1}-\sqrt{\tilde{\alpha}_{\tau-1}}\eta^{i+1}_{0})^2}{1-\tilde{\alpha}_{\tau-1}}\\
%         - \frac{(\eta^{i+1}_{\tau}-\sqrt{\tilde{\alpha}_{\tau}}\eta^{i+1}_{0})^2}{1-\tilde{\alpha}_{\tau}}
%         )  \} \\
%         = exp \{ -\frac{1}{2} ( (\frac{\alpha_\tau}{\beta_\tau} + \frac{1}{1-\tilde{\alpha}}_{\tau-1}) (\mathbf{\eta}^{i+1}_{\tau-1})^2 \\
%         - (2 \frac{\sqrt{\alpha}_\tau}{\beta_\tau} \mathbf{\eta}^{i+1}_{\tau} + 2 \frac{\sqrt{\tilde{\alpha}}_{\tau-1}}{1-\tilde{\alpha}_{\tau-1}} \mathbf{\eta}^{i+1}_0]) \mathbf{\eta}^{i+1}_{\tau-1} + C(\mathbf{\eta}^{i+1}_\tau, \mathbf{\eta}^{i+1}_0) )  \}
%     \end{gathered}
% \end{equation}

% Then by inspection, we can obtain $\tilde{\beta}_\tau$ and $\tilde{\mu}_\tau(\mathbf{\eta}^{i+1}_\tau, \mathbf{\eta}^{i+1}_0)$ as follows:

% \begin{equation}
%     \begin{gathered}
%         \tilde{\beta}_\tau = 1/(\frac{\alpha_\tau}{\beta_\tau} + \frac{1}{1-\tilde{\alpha}_{\tau-1}}) = \frac{1-\tilde{\alpha}_{\tau-1}}{1-\tilde{\alpha}_\tau} \beta_\tau, \\
%         \tilde{\mu}_\tau(\mathbf{\eta}^{i+1}_\tau, \mathbf{\eta}^{i+1}_0) = (\frac{\sqrt{\alpha_\tau}}{\beta_\tau} \mathbf{\eta}^{i+1}_{\tau} + \frac{\sqrt{\tilde{\alpha}_{\tau-1}}}{1-\tilde{\alpha}_{\tau-1}} \mathbf{\eta}^{i+1}_0)/(\frac{\alpha_\tau}{\beta_\tau} + \frac{1}{1-\tilde{\alpha}_{\tau-1}}), \\
%         = \frac{\sqrt{\alpha_\tau}(1-\tilde{\alpha}_{\tau-1})}{1-\tilde{\alpha}_\tau} (\phi^i \mathbf{\eta}^i_\tau + (1-\phi^i) o(\mathbf{H}^i_\tau)) + \frac{\sqrt{\tilde{\alpha}_{\tau-1}}\beta_\tau}{1-\tilde{\alpha}_\tau} \mathbf{\eta}^{i+1}_0.
%     \end{gathered}
% \end{equation}

\begin{equation}
    \begin{gathered}
        \tilde{\beta}_\tau = \frac{1-\tilde{\alpha}_{\tau-1}}{1-\tilde{\alpha}_\tau} \beta_\tau, \\
       \tilde{\mu}_\tau(\mathbf{\eta}^{i+1}_\tau, \mathbf{\eta}^{i+1}_0) = \frac{1}{\sqrt{\alpha_\tau}} (\phi^i \mathbf{\eta}^i_\tau + (1-\phi^i) o(\mathbf{H}^i_\tau) - 2 \frac{1-\alpha_\tau}{\sqrt{1-\tilde{\alpha}_\tau}}\epsilon_\tau),
    \end{gathered}
\end{equation}
which is the closed-form solution of the denoising process.

\subsubsection{Modified Unet}

To effectively model the above code prediction dynamics from $i$-th to $i+1$-th visit, we adopt a U-Net architecture that captures the code-level details, with the guidance of extra information. We denote the feature at $l$-th layer of U-Net as $\mathbf{\eta}^i_l$. The extra information vectors are stacked as $\mathbf{H}^i_l = [\mathbf{h}^i, \mathbf{\Delta \hat{t}^i}, \mathbf{De}, \mathbf{Un}]$ and condensed by an MLP to fit the $l$-th level's dimension of the U-Net. $\mathbf{Un}$ serves as an unknown vector of noise which introduces variety to the generated codes. Aligning with the assumption that $\phi^i \mathbf{\eta}^{i}_{\tau}+ (1-\phi^i) o(\mathbf{H}^{i}_{\tau}) = \mathbf{\eta}^{i+1}_{\tau}$, the skip connection is modified by cross attention with $\mathbf{\eta}^i_l$ and $\mathbf{H}^i_l$ so that the generation is guided while the unwanted information can be filtered:

\begin{equation}
    \mathbf{\eta}^{i+1}_l = \text{CrossAttn}(\mathbf{\eta}^i_l,\mathbf{H}^i_l).
\end{equation}
The reconstructed sample from the U-Net is denoted as $\mathbf{\hat{\eta}}^i_{u,m}$.
% With $\theta$, we are approximating:

% \begin{equation}
%     \mu_\theta(\mathbf{\eta}^{i}_\tau, \tau, \mathbf{H}) = \frac{1}{\sqrt{\alpha}_\tau} (\phi^i \mathbf{\eta}^i_\tau + (1-\phi^i) o(\mathbf{H}^i_\tau) - 2 \frac{1-\alpha_\tau}{\sqrt{1-\tilde{\alpha}_\tau}}\epsilon_\theta(\mathbf{\eta}^{i}_\tau, \tau, \mathbf{H}))
% \end{equation}

\subsubsection{Predicting Codes for Each Modality}
After generating the embeddings for each modality within the visit, we aggregate these embeddings separately for each modality to form distinct modality-specific visit embeddings:

\begin{equation}
    \mathbf{\hat{v}}^i_{u} = \sum_{m=1}^{M_{U}} \mathbf{\hat{\eta}}^i_{u,m},
\end{equation}
where $\mathbf{\hat{\eta}}^i_{u,m}$ represents the generated embedding. We then use a distinct output layer for each modality to predict the respective codes:

\begin{equation}
    \mathbf{\hat{c}}^i_{u} = \text{Sigmoid}(\mathbf{W}_{c_{u}} \mathbf{\hat{v}}^i_{u} + \mathbf{b}_{c_{u}}).
\end{equation}
Here, \(\mathbf{\hat{c}}^i_{\text{mod}}\) represents the predicted codes for the modality $u$. $\mathbf{W}_{c_{u}} \in \mathbb{R}^{M_u*d}$ and $\mathbf{b}_{c} \in \mathbb{R}^{M_u}$ are the weights and biases of the output layer specific to each modality, 

\subsection{Loss Functions}

For the diffusion module, we have $\mathcal{L}_{D}$ that calculates the difference between the real visit and the reconstructed visit as:
\begin{equation}
    \begin{gathered}
        \mathcal{L}_{D} = E_{\mathbf{\eta}^{i+1}_0,\epsilon} [\frac{1}{2||\Sigma||^2}] |\tilde{\mu}_\tau(\mathbf{\eta}^{i+1}_\tau, \mathbf{\eta}^{i+1}_0) -\mu_\theta(\mathbf{\eta}^{i}_\tau, \tau, \mathbf{H})|^2 \\
        = E_{\mathbf{\eta}^{i+1}_0,\epsilon} [C \cdot 2 |\epsilon_\tau - \epsilon_\theta (\mathbf{\eta}^{i}_\tau, \tau, \mathbf{H})|^2].
    \end{gathered}
\end{equation}
For the time gap predictor, we take the Mean Squared Error (MSE) loss $\mathcal{L}_{T}$ of the real time gap and the predicted time gap for all $P$ patients in the training set as:
\begin{equation}
\begin{gathered}
\mathcal{L}_{T} = MSE(\Delta t^i_p, \Delta \hat{t}^i_p),
\end{gathered}
\end{equation}
For the predicted code probabilities in each modality, we utilize the Focal Loss $\mathcal{L}_{F}$ as follows:

\begin{equation}
\begin{gathered}
\mathcal{L}_{F} = -\sum_{u} \sum_{m=1}^{M_{u}} [ c^i_{u,m} F_{\alpha} (1 - \hat{c}^i_{u,m})^{F_{\gamma}} \log(\hat{c}^i_{u,m}) \\
+ (1 - c^i_{u,m})(1 - F_{\alpha}) (\hat{c}^i_{u,m})^{F_{\gamma}} \log(1 - \hat{c}^i_{u,m}) ].
\end{gathered}
\end{equation}
Here,  $c^i_{u,m}$  represents the true code labels for the $m$-th code in the modality $u$ for the $i$-th visit and $F_{\alpha}$ and $F_{\gamma}$ are the hyperparameters for the Focal Loss.

Finally, the total Loss $\mathcal{L}$ is then calculated by:

\begin{equation}
    \mathcal{L} = \lambda_D \mathcal{L}_{D} + \lambda_T log(\mathcal{L}_{T}) + \lambda_F \mathcal{L}_{F},
\end{equation}
where $\lambda_D$, $\lambda_T$, and $\lambda_F$ are hyperparemeters of weighting.


==> files/3-model.tex <==
\section{Preliminary: Diffusion Model}
In this section, we briefly touch on the main components and mechanics of the Denoising Diffusion Probabilistic Model (DDPM).

\subsection{Forward Diffusion Process}
With an input matrix $\mathbf{x}_0$ and a pre-defined variance schedule $\beta_t$, the forward diffusion process gradually adds noise to the original image according to the diffusion time step $t\in(1,T)$ as follows:

\begin{equation}
\begin{gathered}
    q(\mathbf{x}_t|\mathbf{x}_{t-1}) = \mathcal{N}(\mathbf{x}_t;\sqrt{1-\beta_t} \mathbf{x}_{t-1},\beta_t\mathbf{I}),\\
    q(\mathbf{x}_{1:T}|\mathbf{x}_0) = \prod_{t=1}^T q(\mathbf{x}_t|\mathbf{x}_{t-1}).
\end{gathered}
\label{eq:forward}
\end{equation}

Let $\alpha_t = 1-\beta_t$ and $\bar{\alpha}_t = \prod_{i=1}^t\alpha_i$, we can reparametrize the above Gausssian Steps in Eq.\ref{eq:forward} to obtain close form solution of noised image $\mathbf{x}_t$ at any time $t$ without adding noise step by step:

\begin{equation}
    \mathbf{x}_t = \sqrt{\alpha_t} \mathbf{x}_{t-1} + \sqrt{1-\alpha_t}\epsilon_{t-1} = \sqrt{\bar{\alpha}_t} \mathbf{x}_0 + \sqrt{1-\bar{\alpha}_t}\epsilon.
\label{eq:forwardRepa}
\end{equation}

\subsection{Backward Diffusion Process}
The backward diffusion process aims to reverse the above forward process and sample from $q(\mathbf{x_{t-1}|x_t})$ to recreate the true sample. Conditional on $\mathbf{x}_0$, the backward process is Gaussian distributed and can be written in terms of forward diffusion by Bayes Theorem as follows:

\begin{equation}
\begin{gathered}
        q(\mathbf{x}_{t-1}|\mathbf{x}_t,\mathbf{x}_0) = \mathcal{N}(\mathbf{x_{t-1}};\hat{\mu}(\mathbf{x}_t,\mathbf{x}_0),\hat{\beta}_T\mathbf{I}), \\
        q(\mathbf{x}_{t-1}|\mathbf{x}_t,\mathbf{x}_0) = q(\mathbf{x}_t|\mathbf{x}_{t-1},\mathbf{x}_0)\frac{q(\mathbf{x}_{t-1}|\mathbf{x}_0)}{q(\mathbf{x}_t|\mathbf{x}_0)}.
\end{gathered}
\label{eq:backward}
\end{equation}
Then according to the Gaussian distribution's density function, we can obtain the variance $\hat{\beta}_t$ and mean $\hat{\mu}_t(\mathbf{x}_t,\mathbf{x}_0)$  of $q(\mathbf{x}_{t-1}|\mathbf{x}_t,\mathbf{x}_0)$ as:

% \begin{equation}
% \begin{gathered}
%     q(\mathbf{x}_{t-1}|\mathbf{x}_t,\mathbf{x}_0) \propto \\ \text{exp}(-\frac{1}{2}(\frac{(\mathbf{x}_t-\sqrt{\alpha_t}\mathbf{x}_{t-1})^2}{\beta_t}+\frac{(\mathbf{x}_{t-1}-\sqrt{\bar{\alpha}_{t-1}}\mathbf{x}_{0})^2}{1-\bar{\alpha}_{t-1}} - \frac{(\mathbf{x}_t-\sqrt{\bar{\alpha}_t}\mathbf{x}_{0})^2}{1-\bar{\alpha}_{t}})) \\
%     = \text{exp} (-\frac{1}{2}((\frac{\alpha_t}{\beta_t}+\frac{1}{1-\bar{\alpha}_{t-1}})    \mathbf{x}^2_{t-1} - (\frac{2\sqrt{\alpha_t}}{\beta_T}\mathbf{x}_t+\frac{2\sqrt{\bar{\alpha}_{t-1}}}{1-\bar{\alpha}_{t-1}}\mathbf{x}_0)\mathbf{x}_{t-1} + \mathbf{C} )  ),
% \end{gathered}
% \label{eq:mixureGaussian}
% \end{equation}
% where $\mathbf{C}$ is a constant term.

\begin{equation}
    \begin{gathered}
        \hat{\beta}_t 
        % = 1/(\frac{\alpha_t}{\beta_t}+\frac{1}{1-\bar{\alpha}_{t-1}})
        =\frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_t}\beta_t,\\
        \hat{\mu}_t(\mathbf{x}_t,\mathbf{x}_0) 
        % = (\frac{\sqrt{\alpha_t}}{\beta_T}\mathbf{x}_t+\frac{\sqrt{\bar{\alpha}_{t-1}}}{1-\bar{\alpha}_{t-1}}\mathbf{x}_0)/(\frac{\alpha_t}{\beta_t}+\frac{1}{1-\bar{\alpha}_{t-1}}) \\
        =\frac{\sqrt{\alpha}_t(1-\bar{\alpha}_{t-1})}{1-\bar{\mathbf{\alpha}_t}}  \mathbf{x}_t+ \frac{\sqrt{\bar{\alpha}_{t-1}}\beta_t}{1-\bar{\alpha}_t}\mathbf{x}_0.
    \end{gathered}
\label{eq:meanAndVar}
\end{equation}
Substitute Eq.~\ref{eq:forwardRepa} to the above equation, we have the closed-form solution to the backward diffusion process's mean:

\begin{equation}
    \hat{\mu}_t(\mathbf{x}_t,\mathbf{x}_0) = \frac{1}{\sqrt{\alpha}_t}(\mathbf{x}_t - \frac{1-\alpha_t}{\sqrt{1-\bar{\alpha}_t}}\epsilon_t).
\label{eq:meanAndVarofModel1}
\end{equation}
In practice, one can train a neural network $g$ with parameters $\theta$ to approximate Eq.~\ref{eq:meanAndVarofModel1} as $\mu_\theta(\mathbf{x}_t,t)$:

\begin{equation}
    \mu_\theta(\mathbf{x}_t,t) = \frac{1}{\sqrt{\alpha}_t}(\mathbf{x}_t - \frac{1-\alpha_t}{\sqrt{1-\bar{\alpha}_t}}\epsilon_\theta(\mathbf{x}_t,t)).
\label{eq:meanAndVarofModel2}
\end{equation}

\subsection{Loss Function}

The diffusion loss $\mathcal{L}_D$ aims to minimize the difference between close form mean $\hat{\mu}_t(\mathbf{x}_t,\mathbf{x}_0)$ and approximated mean $\mu_\theta(\mathbf{x}_t,t)$, which can be simplified into calculating the difference of added noise $\epsilon_t$ and the learned noise $\epsilon_\theta(\mathbf{x}_t,t)$:

\begin{equation}
    \begin{gathered}
        \mathcal{L}_D = \mathbb{E}||\hat{\mu}_t(\mathbf{x}_t,\mathbf{x}_0)-\mu_\theta(\mathbf{x}_t,t)||^2 
        = \mathbb{E}||\epsilon_t - \epsilon_\theta(\mathbf{x}_t,t))||^2.
    \end{gathered}
\label{eq:ogDiffLoss}
\end{equation}

\subsection{Longitudinal EHR Data Generation with Diffusion Model}

In the context of EHR data generation, we can adapt the above diffusion model $g$ with loss term in Eq.~\ref{eq:ogDiffLoss} to perform visit-level generation in a self-supervised manner. It can be written as $\hat{\mathbf{v}}^i = g(\mathbf{v}^i)$, where $\mathbf{v}^i$ is the representation of the patient's $i$-th original visit and the $\hat{\mathbf{v}}^i$ is the generated result. We will explain the construction of visit embedding $\mathbf{v}$ in Section~\ref{visitemb}. However, this approach ignores some fundamental characteristics of EHR data, such as the time gap between visits and code appearance pattern. These characteristics contain hidden disease progression information and modeling such information is crucial for generating realistic EHR data. To this end, we propose \ours that aims to generate the next visit by the current visit, conditional on the time gap and historical records.

% \subsection{Diffusion Model for EHR Data Generation}

% In recent years, the Denoising Diffusion Probabilistic Model (DDPM) and its variants~\cite{glide,scalable} are among the top most researched and utilized models and have shown great success in data generation tasks. In pursuing a better method to generate realistic EHR data, a few works have adopted the diffusion model to generate tabular form data~\cite{tabddpm} or perform task-oriented data augmentation~\cite{meddiffusion}. Denoting the original visit of the patient's EHR data as $v^i$, existing methods aim to generate a synthetic visit ${v^i}'$ using DDPM as a generation module. They mainly differ from the representation learning and fusion procedures before feeding $v^i$ to DDPM.

% In our course of research~\cite{dipole, medskim, meddiffusion}, we notice that the temporal dynamics is a crucial factor, and the existing EHR data generation models either ignore this factor or do not utilize it efficiently. To find a better approach to modeling the longitudinal EHR data and generate more realistic synthetic data, we propose to shift the generation target from $v^i$ to $v^{i+1}$ instead, i.e., using current visit $v^i$ to generate synthetic next visit ${\hat{v}^{i+1}}$. To cope with our generation target, we need to make modifications to the DDPM.

\section{Methodology}

In this section, we discuss the main components of \ours.

% The proposed \ours comprises four main components for enhanced medical visit prediction: 1) "Synchronized Noise Trajectory" for smooth transitions between visits, 2) "Code-time Dynamics Learner" for detailed temporal analysis of patient condition changes, 3) "Conditional Information Learner" for incorporating various additional data for context, and 4) "MedSyncD-Unet," a specialized U-Net for accurate next visit predictions using this extra information.

% \subsection{Sequential Visit Generation Task}

% As described in the preliminary section, one can adopt the original DDPM to the healthcare domain and generate synthetic data based on real data. For instance, under the setting of longitudinal EHR data generation and denoting the generation model as function $g$, we can write the generation process as $\hat{\mathbf{v}}^i = g(\mathbf{v}^i)$, where $\mathbf{v}$ is a representation of patient's $i$-th original visit and $\hat{\mathbf{v}}^i$ is the generated result. We will explain the construction of visit embedding $\mathbf{v}$ in Section~\ref{visitemb}. However, this approach ignores some fundamental characteristics of EHR data, such as the time gap between visits and code appearance pattern. These characteristics might contain hidden disease progression information and modeling such information is crucial for generating realistic EHR data. Thus we propose \ours to capture and model such information and generate synthetic EHR data with better quality. In summary, our goal is to construct model $g$ to predict on the next $i+1$-th visit $\mathbf{v}^{i+1}$ with current visit $\mathbf{v}^i$: $\hat{\mathbf{v}}^{i+1} = g(\mathbf{v}^{i})$.

\subsection{Noise Addition and Visit Reconstruction}\label{main}

For two consecutive visits embedding $\mathbf{v}^i_0$ and $\mathbf{v}^{i+1}_0$ of the same patient, we can obtain their noise addition trajectory separately following Eq.~\ref{eq:forwardRepa}. As the diffusion time step $t\to \infty$, both $\mathbf{v}^i_T$ and $\mathbf{v}^{i+1}_T$ converge to the same Gaussian Distribution $\mathcal{N}\sim (0,\mathbf{I})$ and become indistinguishable: $\mathbf{v}^i_T \approx \mathbf{v}^{i+1}_T$. Since both visits come from the same sample space and contain similar information, we speculate that there exists a function $f$ that can describe their relation at each intermediate diffusion time step $t \in (1, T-1)$, as follows:

\begin{equation}
    \mathbf{v}^{i+1}_t = f(\mathbf{v}^i_t, \mathbf{H}^i),
\label{eq:syncD}
\end{equation}
where $\mathbf{H}^i$ is an embedding matrix of extra information that function $f$ conditions on and will be explained in detail in Section~\ref{conditionalemb}. This relation is visualized in the center of Figure~\ref{fig:mainplot}. Then by Eq.~\ref{eq:meanAndVarofModel1} in the backward diffusion process of denoising $\mathbf{v}^{i+1}_t$, we can obtain the mean and variance reparametrized by Eq.~\ref{eq:syncD} as follows:
% This Eq.~\ref{eq:syncD} describes a synchronization of noise trajectory of $\mathbf{v}^i_t$ and $\mathbf{v}^{i+1}_t$ that is bridged by $\mathbf{H}^i$ so we name it Synchronized Noise Trajectory, as shown in Figure~\ref{fig:unetplot}. 

\begin{figure*}[]
    \centering
    \includegraphics[width=0.90\textwidth]{figure/mainplot.pdf}
    \vspace{-2mm}
    \caption{Overview of the proposed {\ours} model.}
    \label{fig:mainplot}
\end{figure*}

\begin{equation}
\begin{gathered}
\hat{\beta}_t = \frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_t} \beta_t, \\
\hat{\mu}_t(\mathbf{v}^{i+1}_t, \mathbf{v}^{i+1}_0) = \frac{1}{\sqrt{\alpha_t}} (f(\mathbf{v}^i_t, \mathbf{H}^i)- \frac{1-\alpha_t}{\sqrt{1-\bar{\alpha}_t}}\epsilon_t).
\end{gathered}
\end{equation}
By this construction, we can use $f(\mathbf{v}^i_t, \mathbf{H}^i)$ as the noisy input instead of $\mathbf{v}^{i+1}_t$ and rewrite the generating function $g$ as follows: $\hat{\mathbf{v}}^{i+1} = g(f(\mathbf{v}^i_t, \mathbf{H}^i))$. In the next section, we will introduce our generation module that achieves this step-wise generation purpose.
% We further propose MedSyncD-Unet as the generation module $g$ in Section~\ref{unet} to achieve the generation purpose

\subsection{Step-wise Visit Generation Module}\label{unet}

The conventional U-Net architecture is primarily designed for 2-dimensional input, lacking components to handle the sequential characteristics of the longitudinal EHR data. To address this issue, we introduce the step-wise visit generation module $g$, which is adept at generating the next visit prediction $\hat{\mathbf{v}}^{i+1}$ from the current visit $\mathbf{v}^i_t$, conditioned on the historical context $\mathbf{H}^i$. We illustrate its architecture in the right side of Figure~\ref{fig:mainplot}.

In our architecture, $l$ represents the layer number in U-Net, such as $\mathbf{v}^i_{l,t}$. Within the $l$-th layer of the downsampling path, we utilize a Resnet block with a 1-dimensional convolution layer for feature learning and a downsampling layer for compressing features:

\begin{equation}
    \begin{gathered}
        ResnetBlock(\mathbf{v}^{i+1}_{l,t}) = \mathbf{v}^{i+1}_{l,t} + ConvBlock(\mathbf{v}^{i+1}_{l,t}),\\
        \mathbf{v}^{i+1}_{l+1,t} = Downsample(ResnetBlock(\mathbf{v}^{i+1}_{l,t})).
    \end{gathered}
\end{equation}

For the upsampling path, a transformer encoder block at the $l$-th level performs the embedding fusion of $\mathbf{v}^{i+1}_{l}$ and $\mathbf{H}^{i}$, achieving the function $f$ in Eq.~\ref{eq:syncD}. Here, the $l$-th level of $\mathbf{H}^{i}_l$ is resized through a linear layer to match the dimension of $\mathbf{v}^{i+1}_{l}$. The cross-attention fusion is expressed as:
\begin{equation}
\begin{gathered}
\bar{\mathbf{v}}^{i+1}_{l,t} = Softmax\left(\frac{\mathbf{W}^Q_l(\mathbf{v}^{i+1}_{l,t})\cdot\mathbf{W}^K_l(\mathbf{H}^i_l)}{\sqrt{d}}\right)\cdot\mathbf{W}^V_l(\mathbf{H}^i_l),\\
\mathbf{v}^{i+1}_{l,t} = MaxPooling(LayerNorm(\mathbf{v}^{i+1}_{l,t}) + \bar{\mathbf{v}}^{i+1}_{l,t}),
\end{gathered}
\end{equation}
where $\mathbf{W}^Q_l, \mathbf{W}^K_l, \mathbf{W}^V_l \in \mathbb{R}^{d*d}$.

Subsequently, the $l$-th layer in the upsampling path fuses the skip connection output with features from the $(l+1)$-th layer:

\begin{equation}
\begin{gathered}
\mathbf{v}^{i+1}_{l,t} = ResnetBlock(\mathbf{v}^{i+1}_{l,t} + ConvBlock([\mathbf{v}^{i+1}_{l,t},\mathbf{v}^{i+1}_{l+1,t}]))
\end{gathered}
\end{equation}

The final output, $\mathbf{v}^{i+1}_{0,0}$, is the reconstructed visit $\hat{\mathbf{v}}^{i+1}$, that contains the subsequent visit's informaion.

\subsubsection{Loss Function of MedSyncD-Unet}

Similar to Eq.~\ref{eq:ogDiffLoss}, we have $\mathcal{L}_{D}$ that calculates the reconstruction loss as:
\begin{equation}
    \begin{gathered}
        \mathcal{L}_{D} = \mathbb{E} ||\hat{\mu}_t(\mathbf{v}^{i+1}_t, \mathbf{v}^{i+1}_0) -\mu_\theta(\mathbf{v}^{i}_t,t, \mathbf{H}^i)||^2 \\
        = \mathbb{E} ||\epsilon_t - \epsilon_\theta (\mathbf{v}^{i}_t, t, \mathbf{H}^i)||^2.
    \end{gathered}
\end{equation}

\subsubsection{Medical Codes Prediction}

With the generated visit $\hat{\mathbf{v}}^{i+1}$, we utilize an linear layer to output medical codes:

\begin{equation}
    \mathbf{\hat{c}}^{i+1} = \text{Sigmoid}(\mathbf{W}_{c} \mathbf{\hat{v}}^{i+1} + \mathbf{b}_{c}).
\end{equation}
Here, $\mathbf{\hat{c}}^{i+1}$ represents the predicted codes. $\mathbf{W}_{c} \in \mathbb{R}^{M*d}$ and $\mathbf{b}_{c} \in \mathbb{R}^{M}$ are the weights and biases of the output layer.

\subsubsection{Loss Function of Predicted Codes}

We utilize the Focal Loss to calculate code prediction loss $\mathcal{L}_{F}$ as follows:

\begin{equation}
\begin{gathered}
\mathcal{L}_{F} = -\sum_{m=1}^{M} [ c^i_{m} F_{\alpha} (1 - \hat{c}^i_{m})^{F_{\gamma}} \log(\hat{c}^i_{m}) \\
+ (1 - c^i_{m})(1 - F_{\alpha}) (\hat{c}^i_{m})^{F_{\gamma}} \log(1 - \hat{c}^i_{m}) ].
\end{gathered}
\end{equation}
Here,  $c^i_{m}$  represents the true code labels for the $m$-th code for the $i$-th visit, and $F_{\alpha}$ and $F_{\gamma}$ are the hyperparameters for the Focal Loss.

\subsection{Code-level Dynamics Learning Module} \label{visitemb}

In the previous section, we extensively utilize $\mathbf{v}^i$ as the visit embedding. Conventionally, for the $m$-th code in a patient's $i$-th visit, an embedding layer can be used to transform it into dense embedding $\mathbf{c}_{m}$ of dimension $d$. Then the visit level embedding $\mathbf{v}^i$ can be obtained by taking summation along code dimension $m$. However, the visit embedding obtained with this approach is static and doesn't encapsulate the temporal evolution of the disease across multiple visits. To address this deficiency, we propose a code-level dynamics learning module, a fine-grained approach to capture the temporal dynamics of each medical code individually, which is detailed in this section. We show the relationship between the time gap and codes in the left part of Figure~\ref{fig:mainplot}. Note that there can be multiple medical code modalities that are processed the same way as described.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\columnwidth]{figure/codetimeplot.png}
%     \caption{Illustration of Medical Codes and Time.}
%     \label{fig:ctplot}
% \end{figure}

\subsubsection{Code Level Time Gap Construction}

% To model the code-time interaction in a fine-grained manner, we first construct code-level time gaps as a feature, based on visit-level time gaps. Denoting the time of the current appearance of the code $m$ as $t^k_m$ and the time of its last appearance as $t^j_m$, the code level time gap is the difference between current appearance against its latest appreance, with its first appreance is always 0 $\Delta t^1_m = 0, \Delta t^j_m = t^k_m - t^j_m, \quad \text{for } j > 1, j < k.$

To capture the intricacies of code-time interactions, we construct a feature representing code-level time gaps, which is derived from the visit level time stamp $t^i$. We define the code-level time gap as the interval between the current and most recent appearances of a specific code $m$. Let $t^k_m$ represent the time of code $m$'s current appearance, and $t^j_m$ denote the time of its last appearance. The code-level time gap is calculated as $\Delta t^j_m = t^k_m - t^j_m, j<k$
, with a condition that the gap for the first appearance is always zero, i.e., \( \Delta t^1_m = 0 \).



% \begin{equation}
%     \begin{gathered}
% \Delta t^1_m = 0 \\
% \Delta t^j_m = t^k_m - t^j_m, \quad \text{for } j > 1, j < k.
%     \end{gathered}
% \end{equation}


\subsubsection{Fine-grained Code-time Embedding:}
For code $c^i_m$, an embedding layer transforms the discrete code into a dense embedding $\mathbf{c}^i_{m}$  of dimension $d$. The code embedding is then merged with the corresponding time gap embedding $\Delta t^i_{m}$ to model the code-time dynamics, forming $\mathbf{\eta}^i_{m}$as follows:

\begin{equation}
\begin{gathered}
    \mathbf{\eta}^i_{m} = o(\mathbf{c}^i_{m}, \mathbf{\Delta t}^i_{m}) \text{MLP}(\mathbf{c}^i_{m}, \mathbf{\Delta t}^i_{m}) + (1- o(\mathbf{c}^i_{m}, \mathbf{\Delta t}^i_{m})) \mathbf{c}^i_{m}.
\end{gathered}
\label{eq:timeEncoding}
\end{equation}
In the above Eq.~\ref{eq:timeEncoding}, $\mathbf{\Delta t}^i_{m}$ is calculated by Positional Embedding. An MLP is used to merge the code and time information. Function $o$ produces a binary output that represents whether the presented code embedding $\mathbf{c}^i_{m}$ should be modified based on the time gap information $\mathbf{\Delta t}^i_{m}$. We employ a Gumbel-Softmax layer to sample from this decision-making process while keeping it differentiable, as shown in Eq.~\ref{eq:gumbel}. 

\begin{equation}
        o(\mathbf{c}^i_{m}, \mathbf{\Delta t}^i_{m}) = \text{Binarize}\left( \frac{\exp\left(\frac{\log(\mathbf{p}^i_{m}[0]) + g_0}{\tau}\right)}{\sum_{j=0}^{1} \exp\left(\frac{\log(\mathbf{p}^i_{m}[j]) + g_j}{\tau}\right)} \right).
\label{eq:gumbel}
\end{equation}

\subsubsection{Aggregated Visit-level Embedding:}
As mentioned in the previous section, our input data could contain different modalities of medical codes. Denoting the modality with $u$, the fine-grained code-time embedding can be rewritten as $\mathbf{\eta}^i_{u,m}$. To dynamically acquire the most relevant information from each modality, we utilize a modality-level attention layer to dynamically aggregate embedding. The process starts by summing the code level information with a feed-forward layer: $\mathbf{z}^i_{u}= \text{ReLU}(\mathbf{W}_{u} \sum_{m=1}^{M_{u}} \mathbf{\eta}^i_{u,m} + \mathbf{b}_{u})$, where $\mathbf{W}_{u}\in \mathbb{R}^{d*d}, \mathbf{d}_{u} \in \mathbb{R}^d$, and $M_{u}$ denotes the total number of codes in modality $u$. Then the attention scores for the modalities are computed as: $\mathbf{s}^i = \text{Softmax}(\mathbf{W}_{s} [\mathbf{z}^i_{1}, \mathbf{z}^i_{2},\cdots, \mathbf{z}^i_{U}] + \mathbf{b}_{s})$, where $\mathbf{W}_{s}\in \mathbb{R}^{U*d} $ and $ \mathbf{b}_{s} \in \mathbb{R}^{d}$. The final visit-level embedding is computed by the weighted sum of embeddings: $\mathbf{v}^i = \mathbf{s}^i_{u} \cdot \mathbf{z}^i_{u}$.

\subsection{Conditional Information Learning Module} \label{conditionalemb}

As the previous section has emphasized, a conditional information matrix $\mathbf{H}^i$ provides crucial information that guides the generation process of \ours. In this section, we describe how we construct $\mathbf{H}^i$ that includes medical history, time gap till the next visit, and demographic information.

\subsubsection{Medical History Learning}

Medical history is one of the most important information that helps forecast the future condition of a patient. With the visit level embedding $\mathbf{v}^i$, we can utilize an LSTM network to accumulate hidden state per visit, as follows: $\mathbf{h}^i = \text{LSTM}(\mathbf{h}^{i-1},\mathbf{v}^i)$.


\subsubsection{Visit-Level Time Gap Prediction}

Another crucial information to consider is the follow-up visit time. In clinical practice, healthcare professionals rely heavily on a patient's medical history and current health indicators to decide the timing of the next follow-up visit, a process vital for effective treatment planning. Our model seeks to mimic this critical aspect of the decision process. In doing so, it addresses a gap in existing Electronic Health Record (EHR) data generation methods~\cite{promptehr,twin}, which typically do not incorporate visit time gap information.

Following the work of continuous-time LSTM with Hawkes Process~\cite{hawkeslstm}, we utilize the hidden state $\mathbf{h}^i$ and employ a two-step linear transformation to predict the visit-level time gap, as shown in Eq.\ref{eq:timepred}. We first utilize a linear layer on hidden state $\mathbf{h}^i$ to learn an intensity measure $\lambda^i(t)$ of the current visit, which represents a patient's medical urgency. This intensity is subtracted from $1$, giving a close to $0$ output if the patient's condition is urgent. Then the second equation predicts the time gap and ensures it is strictly above $0$ with the Softplus activation function:

\begin{equation}
\begin{aligned}
    \mathbf{\lambda^i(t)} &= 1 - \text{tanh}(\mathbf{W}_\lambda \mathbf{h}^i + \mathbf{b}_\lambda),\\
    \Delta \hat{t}^i &= \text{Softplus}(\mathbf{W}_{\hat{t}} \mathbf{\lambda^i(t)} + b_{\hat{t}}).
\end{aligned}
\label{eq:timepred}
\end{equation}
where $\mathbf{W}_\lambda \in \mathbb{R}^{d\times d}; \mathbf{W}_{\hat{t}}$ and $\mathbf{b}_{\lambda} \in \mathbb{R}^d$ ; $ \mathbf{b}_{\hat{t}} \in \mathbb{R}$.

\subsubsection{Loss Function of Predicted Visit-Level Time Gap}

For the time gap predictor, we take the Mean Squared Error (MSE) loss $\mathcal{L}_{T}$ of the real time gap and the predicted time gap for all $P$ patients in the training set as:
\begin{equation}
\begin{gathered}
\mathcal{L}_{T} = MSE(\Delta t^i_p, \Delta \hat{t}^i_p),
\end{gathered}
\end{equation}

\subsubsection{Demographic Information}

Besides the extra information in previous sections, demographic details such as age and sex also play a crucial role. To ensure that information inconsistent with the patient's demographic characteristics is filtered out, we encode these demographics into a multi-hot encoded vector $\mathbf{D}$, and introduce it to our model by embedding it into a dense dimension $d$ using a linear layer: $\mathbf{De} = \mathbf{W}_D\mathbf{D} + \mathbf{b}_D$, where $\mathbf{W}_D \in \mathbb{R}^{d*D}$ and $ \mathbf{b}_D \in \mathbb{R}^d$.

\subsubsection{Extra Information Matrix Construction}

Finally, we can construct the extra information matrix $\mathbf{H}^i$ by concatenation as follows: $\mathbf{H}^i = [\mathbf{h}^i, \mathbf{De}, \Delta \hat{\mathbf{t}}^i]$, where $\Delta \hat{\mathbf{t}}^i \in \mathbf{R}^d$ is the predicted visit-level time gap embedding calculated by Positional Embedding with $\Delta \hat{t}^i$.



\subsection{Loss Function}

Finally, the total Loss $\mathcal{L}$ is the weighted sum of all three loss components by $\lambda_D$, $\lambda_T$, and $\lambda_F$, as follows:

\begin{equation}
    \mathcal{L} = \lambda_D \mathcal{L}_{D} + \lambda_T \mathcal{L}_{T} + \lambda_F \mathcal{L}_{F}.
\end{equation}



% we can utilize model $g$ and replicate this method by generating synthetic $i$-th visit $\hat{\mathbf{v}}^i$ from real visit $\mathbf{v}^i$: $g(\mathbf{v}^i) = \hat{\mathbf{v}}^i$. However, this approach ignores the temporal dynamics of EHR data that contain crucial information such as disease progression and previous medical history. Thus in this section, we propose a novel method that aims to generate $i+1$-th visit $\hat{\mathbf{v}}^{i+1}$ from $\mathbf{v}^i$, with the help of 

% Generating the next visit $v^{i+1}$ with $v^i$ might sound straightforward with an MLP, but it is not the case for the diffusion model. Under the traditional setting with diffusion model $\theta$, a synthetic visit is obtained by ${\hat{v}^i} = \theta(v^i+\epsilon)$, where the model $\theta$ is trained by minimizing the learned noise against added noise from $\mathcal{L}_D = MSE(\epsilon_\theta-\epsilon)$. Then under our new generation setting, our model can be written as ${\hat{v}^{i+1}}=\theta(v^i+\epsilon)$. 

% Starting with visit representation matrix $\mathbf{v}^i$, obtained by embedding methods discussed later, we further denote the diffusion timestep as $\tau$ and the variance schedule as $\beta_\tau$ and $\alpha_\tau = 1-\beta_\tau$. Thus the noise-added trajectory of a patient's visit can be written as $\mathbf{v}^i_{0:T} = [\mathbf{v}^i_0, \cdots,\mathbf{v}^i_\tau,\cdots,\mathbf{v}^i_T]$, where $T$ is the maximum diffusion timestep and $0$ represents the original visit.

% Given two consecutive visit samples $\mathbf{v}^{i}_{0}$ and $\mathbf{v}^{i+1}_0$ of the same patient, we first have the following property during a forward diffusion process:

% \begin{theorem}
% \textbf{Convergence in Forward Diffusion Process:} 
% As the diffusion process progresses ($\tau \to T$), the samples $\mathbf{v}^{i}_{\tau}$ and $\mathbf{v}^{i+1}_{\tau}$ become increasingly similar, converging to a common Gaussian distribution as $T \to \infty$:
% \begin{equation}
%         \lim_{T \to \infty} \mathbf{v}^{i}_{T}, \mathbf{v}{}^{i+1}_{T} \sim \mathcal{N}(0,\mathbf{I}).
% \end{equation}
% \label{theorem1}
% \end{theorem}
% Theorem~\ref{theorem1} gives: $\mathbf{v}^i_0 + \epsilon_T = \mathbf{v}^i_T \approx \mathbf{v}^{i+1}_T$, making it possible to reconstruct $\mathbf{v}^{i+1}_0$ with $\mathbf{v}^{i}_0$. However, this construction purely relies on the diffusion model to capture the consecutive relationship and does not consider historical information at all, leading to suboptimal performance and potential divergence during training. Thus we further modify the diffusion model to generate synthetic visits conditionally on an extra information representation matrix, denoted as $\mathbf{H} \in \mathbb{R}^{d_h*d}$. Specifically, we add $\mathbf{H}$ to the noise addition trajectory of the forward diffusion process and name it Synchronized Noise Addition Trajectory, as follows:
% \begin{theorem}
% \textbf{Synchronized Noise Addition Trajectory:} 
% The noised $i+1$-th code embedding matrix is modeled as the summation of the $i$-th code embedding matrix and additional information matrix $\mathbf{H}^{i}$:
% \begin{equation}
%     \mathbf{v}^{i+1}_{\tau} = \phi^i \mathbf{v}^{i}_{\tau} + (1-\phi^i) \mathbf{H}^{i},
% \end{equation}
% where $\phi^i \in \mathbf{R}^d$ is a learned weighting vector.
% \label{theorem2}
% \end{theorem}

% By Theorem~\ref{theorem2}, we are able to reconstruct $\mathbf{v}^{i+1}_0$ starting at any $\tau \in (1,T)$, conditional on $\mathbf{H}^{i}$. Additionally, the backward diffusion process of denoising $\mathbf{v}^{i+1}_{\tau}$ can be written by the Bayes Theorem:

% \begin{equation}
%     \begin{gathered}
%         q(\mathbf{v}^{i+1}_{\tau-1}|\mathbf{v}^{i+1}_{\tau},\mathbf{v}^{i+1}_{0}) = q(\mathbf{v}^{i+1}_{\tau}|\mathbf{v}^{i+1}_{\tau-1},\mathbf{v}^{i+1}_{0}) \frac{q(\mathbf{v}^{i+1}_{\tau-1}|\mathbf{v}^{i+1}_{0})}{q(\mathbf{v}^{i+1}_{\tau}|\mathbf{v}^{i+1}_{0})}.
%     \end{gathered}
% \end{equation}
% Then we can obtain the mean $\tilde{\beta}_\tau$ and variance $\tilde{\mu}_\tau(\mathbf{v}^{i+1}_\tau, \mathbf{v}^{i+1}_0)$ of the backward process's cumulative distribution by the definition of normal distribution and some simplification, in terms of $\mathbf{v}^i_\tau$: 

% \begin{equation}
%     \begin{gathered}
%         \tilde{\beta}_\tau = \frac{1-\tilde{\alpha}_{\tau-1}}{1-\tilde{\alpha}_\tau} \beta_\tau, \\
%        \tilde{\mu}_\tau(\mathbf{v}^{i+1}_\tau, \mathbf{v}^{i+1}_0) = \frac{1}{\sqrt{\alpha_\tau}} (\phi^i \mathbf{v}^i_\tau + (1-\phi^i) \mathbf{H}^i_\tau - \frac{1-\alpha_\tau}{\sqrt{1-\tilde{\alpha}_\tau}}\epsilon_\tau),
%     \end{gathered}
% \end{equation}
% which is the closed-form solution of the denoising process.


% Similar to the existing works~\cite{tabddpm,meddiffusion}, a go-to solution is to use $\phi^i \mathbf{v}^{i}_{\tau} + (1-\phi^i) \mathbf{H}^{i}$ as the input to the diffusion module. This method treats the input as a direct weighted summation of two modalities. However, this approach is suboptimal in preserving unique features inherent to each modality, which might be lost or diluted if doing so. Thus, we propose the following MedSync-Unet module to handle the reconstruction process. Figure~\ref{fig:unetplot} shows its structure.
% \begin{figure}
    
%     \centering
%     \includegraphics[width=0.8\columnwidth]{figure/unetplots.png}
%     \caption{Illustration of MedSync-Unet}
%     \label{fig:unetplot}
% \end{figure}

==> files/old-tables.tex <==
\begin{table*}[]
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{l|llllllllllll}
Database          & \multicolumn{12}{l}{MIMIC-III}                                                                                                                           \\ \hline
Modality          & \multicolumn{3}{l|}{Diagnosis}         & \multicolumn{3}{l|}{Drug}              & \multicolumn{3}{l|}{Lab}               & \multicolumn{3}{l}{Procedure} \\ \hline
Adacare Backbone  & AUPR & F1 & \multicolumn{1}{l|}{Kappa} & AUPR & F1 & \multicolumn{1}{l|}{Kappa} & AUPR & F1 & \multicolumn{1}{l|}{Kappa} & AUPR     & F1     & Kappa     \\ \hline
Orginal           &0.6310&0.6209&
\multicolumn{1}{l|}{0.4031}      &0.6488&0.6129& \multicolumn{1}{l|}{0.3605}      &0.4683&0.5265& \multicolumn{1}{l|}{0.1613}      & 0.5620&0.5273&0.2870  \\
LSTM+MLP          &0.6640&0.6376& \multicolumn{1}{l|}{0.4185}      &0.6321&0.6000& \multicolumn{1}{l|}{0.3267}      & 0.4983&0.5172 & \multicolumn{1}{l|}{0.2211}      &  0.5873&0.5610&0.2955        \\
LSTM+medGAN       &0.6669&0.6400& \multicolumn{1}{l|}{0.4089}      & 0.6055&0.6032   & \multicolumn{1}{l|}{0.3375}      & 0.5085&0.5211 & \multicolumn{1}{l|}{0.1868}      &  0.5870&0.5447&0.3091    \\
LSTM+TabDDPM      &0.6677&0.6243& \multicolumn{1}{l|}{0.3877}      &      &    & \multicolumn{1}{l|}{}      &      &    & \multicolumn{1}{l|}{}      &          &        &           \\
EVA               &0.6590&0.6424& \multicolumn{1}{l|}{0.4189}      &      &    & \multicolumn{1}{l|}{}      &      &    & \multicolumn{1}{l|}{}      &          &        &           \\
synTEG            &0.6711&0.6121 & \multicolumn{1}{l|}{0.4142}      & 0.6426&0.6084& \multicolumn{1}{l|}{0.3598}      & 0.5108&0.4972  & \multicolumn{1}{l|}{0.2230}      & 0.5736&0.5605&0.3005    \\
PromptEHR         &0.6810&0.6462& \multicolumn{1}{l|}{0.4100}      &      &    & \multicolumn{1}{l|}{}      &      &    & \multicolumn{1}{l|}{}      &          &        &           \\
TWIN              &0.6739&0.6252 & \multicolumn{1}{l|}{0.4328}      &  0.5903&0.5757 & \multicolumn{1}{l|}{0.2985}      & 0.5096&0.5120& \multicolumn{1}{l|}{0.2397}      &  0.5866& 0.5644&0.3055 \\ \hline
Ours              &\textbf{0.6856}&\textbf{0.6523} & \multicolumn{1}{l|}{\textbf{0.4385}}      &  \textbf{0.6597}&\textbf{0.6131} & \multicolumn{1}{l|}{\textbf{0.3693}}      & \textbf{0.5269}&\textbf{0.5363} & \multicolumn{1}{l|}{\textbf{0.2610}}      & \textbf{0.5908}&\textbf{0.5739}&\textbf{0.3110} \\ \hline

Dipole Backbone   & AUPR & F1 & \multicolumn{1}{l|}{Kappa} & AUPR & F1 & \multicolumn{1}{l|}{Kappa} & AUPR & F1 & \multicolumn{1}{l|}{Kappa} & AUPR     & F1     & Kappa     \\ \hline
Orginal           &0.6774&0.6425& \multicolumn{1}{l|}{0.4386}      &  0.6589&0.5962& \multicolumn{1}{l|}{\textbf{0.4089}}      & 0.5133&0.4715& \multicolumn{1}{l|}{0.2204}      &   0.5823&0.5560&0.3246 \\
LSTM+MLP          &0.6872&0.6470 & \multicolumn{1}{l|}{0.4511}      & 0.6659&0.5927 & \multicolumn{1}{l|}{0.3965}      & 0.5169&0.4729& \multicolumn{1}{l|}{0.2014}      &  \textbf{0.6173}&0.5516&0.3085 \\
LSTM+medGAN       &0.6915&0.6371& \multicolumn{1}{l|}{0.4490}      &0.6745&0.5830& \multicolumn{1}{l|}{0.3669}      & 0.5231&0.4981& \multicolumn{1}{l|}{0.2284}      &  0.6109&0.5341&0.3080 \\
LSTM+TabDDPM      &0.6851&0.6342& \multicolumn{1}{l|}{0.4312}      &      &    & \multicolumn{1}{l|}{}      &      &    & \multicolumn{1}{l|}{}      &          &        &           \\
EVA               &0.6795&0.6527& \multicolumn{1}{l|}{0.4513}      &      &    & \multicolumn{1}{l|}{}      &      &    & \multicolumn{1}{l|}{}      &          &        &           \\
synTEG            &0.6820&0.6215& \multicolumn{1}{l|}{0.4174}      &0.6885&0.5927& \multicolumn{1}{l|}{0.3964}      & 0.5295&0.5087& \multicolumn{1}{l|}{0.2532}      &  0.6038&0.5306&0.3091 \\
PromptEHR         &0.6748&0.6359& \multicolumn{1}{l|}{0.4334}      &      &    & \multicolumn{1}{l|}{}      &      &    & \multicolumn{1}{l|}{}      &          &        &           \\
TWIN              &0.6603&0.6409& \multicolumn{1}{l|}{0.4406}      &0.6691&0.6020& \multicolumn{1}{l|}{0.3920}      & 0.5249&0.5085& \multicolumn{1}{l|}{0.2467}      & 0.6043&0.5636&0.3155  \\ \hline
Ours              &  \textbf{0.7018}&\textbf{0.6630}& \multicolumn{1}{l|}{\textbf{0.4735}}      &\textbf{0.6997}&\textbf{0.6069}& \multicolumn{1}{l|}{0.3993}      & \textbf{0.5348}&\textbf{0.5281}& \multicolumn{1}{l|}{\textbf{0.2715}}      & 0.6149&\textbf{0.5671}&\textbf{0.3351} \\ \hline

HiTANet Backbone  & AUPR & F1 & \multicolumn{1}{l|}{Kappa} & AUPR & F1 & \multicolumn{1}{l|}{Kappa} & AUPR & F1 & \multicolumn{1}{l|}{Kappa} & AUPR     & F1     & Kappa     \\ \hline
Orginal           &0.6203&0.5978& \multicolumn{1}{l|}{0.3740}& 0.5667&0.5895& \multicolumn{1}{l|}{0.3542}      & 0.5005&0.4963& \multicolumn{1}{l|}{0.2177}      &  0.6064&0.5720&0.3578  \\
LSTM+MLP          &0.6692&0.6562& \multicolumn{1}{l|}{0.4488}& 0.6443&0.5927& \multicolumn{1}{l|}{0.3684}      &0.5327&0.4960& \multicolumn{1}{l|}{0.2427}      & 0.5715&0.5673&0.3212 \\
LSTM+medGAN       &0.6781&0.6492& \multicolumn{1}{l|}{0.4376}      &0.6544&0.6024& \multicolumn{1}{l|}{0.3522}      &0.5292&0.5048& \multicolumn{1}{l|}{0.2474}      &0.6029&0.5703&0.3421\\
LSTM+TabDDPM      &0.6633&0.6581& \multicolumn{1}{l|}{0.4480}      &      &    & \multicolumn{1}{l|}{}      &      &    & \multicolumn{1}{l|}{}      &          &        &           \\
EVA               &0.6813&0.6511& \multicolumn{1}{l|}{0.4372}      &      &    & \multicolumn{1}{l|}{}      &      &    & \multicolumn{1}{l|}{}      &          &        &           \\
synTEG            &0.6851&0.6607& \multicolumn{1}{l|}{0.4641}      &0.6515&0.5795& \multicolumn{1}{l|}{0.3071}      &0.5323&0.4990& \multicolumn{1}{l|}{\textbf{0.2634}}      &   0.6108&0.5551&0.3451 \\
PromptEHR         &0.6541&0.6182& \multicolumn{1}{l|}{0.4076}      &      &    & \multicolumn{1}{l|}{}      &      &    & \multicolumn{1}{l|}{}      &          &        &           \\
TWIN              &0.6789&0.6690 & \multicolumn{1}{l|}{0.4274}   &0.6458&0.5986& \multicolumn{1}{l|}{0.3536}      & 0.4820&0.4329& \multicolumn{1}{l|}{0.1566}      & 0.6108&0.5786&0.3092  \\ \hline
Ours              &\textbf{0.7017}&\textbf{0.6777}& \multicolumn{1}{l|}{\textbf{0.4699}}      &\textbf{0.6689}&\textbf{0.6092}& \multicolumn{1}{l|}{\textbf{0.3763}}      & \textbf{0.5368}&\textbf{0.5081}& \multicolumn{1}{l|}{0.2484}      &\textbf{0.6159}&\textbf{0.5977}&\textbf{0.3689}\\ \hline

LSTM Backbone     & AUPR & F1 & \multicolumn{1}{l|}{Kappa} & AUPR & F1 & \multicolumn{1}{l|}{Kappa} & AUPR & F1 & \multicolumn{1}{l|}{Kappa} & AUPR     & F1     & Kappa     \\ \hline
Orginal           &0.6549&0.6036& \multicolumn{1}{l|}{0.4119}      & 0.6556&0.5784& \multicolumn{1}{l|}{0.3787}      &0.4985&0.4222& \multicolumn{1}{l|}{0.1902}      & 0.5887&0.5533&0.3096\\
LSTM+MLP          &0.6706&0.6374& \multicolumn{1}{l|}{0.4460}      & 0.6427&0.5809& \multicolumn{1}{l|}{0.3671}      & 0.4783&0.4562 & \multicolumn{1}{l|}{0.1987}      & 0.6017&0.5383&0.3058 \\
LSTM+medGAN       &0.6667&0.6332& \multicolumn{1}{l|}{0.4431}      &0.6422&0.6045& \multicolumn{1}{l|}{0.3882}      &0.5010&\textbf{0.4706}& \multicolumn{1}{l|}{0.2031}      &0.6016&0.5367&0.3284\\
LSTM+TabDDPM      &0.6687&0.6317& \multicolumn{1}{l|}{0.4301}      &      &    & \multicolumn{1}{l|}{}      &      &    & \multicolumn{1}{l|}{}      &          &        &           \\
EVA               &0.6629&0.6307& \multicolumn{1}{l|}{0.4267}      &      &    & \multicolumn{1}{l|}{}      &      &    & \multicolumn{1}{l|}{}      &          &        &           \\
synTEG            &0.6676&0.6312& \multicolumn{1}{l|}{0.4353}      &0.6448&0.5957& \multicolumn{1}{l|}{0.3869}      &0.5000&0.4258& \multicolumn{1}{l|}{0.1798}      &  0.6052&0.5560&0.3259\\
PromptEHR         &0.6642&0.6222& \multicolumn{1}{l|}{0.4178}      &      &    & \multicolumn{1}{l|}{}      &      &    & \multicolumn{1}{l|}{}      &          &        &           \\
TWIN              &0.6546&0.6264& \multicolumn{1}{l|}{0.4162}      & 0.6532&0.5840& \multicolumn{1}{l|}{0.3643}      &0.5040&0.4468& \multicolumn{1}{l|}{0.2049}      & 0.6010&0.5427&0.3305\\ \hline
Ours              &\textbf{0.6824}&\textbf{0.6484}& \multicolumn{1}{l|}{\textbf{0.4506}}      &\textbf{0.6710}&\textbf{0.6064}& \multicolumn{1}{l|}{\textbf{0.3942}}      &\textbf{0.5186}&0.4511& \multicolumn{1}{l|}{\textbf{0.2110}}      &\textbf{0.6156}&\textbf{0.5644}&\textbf{0.3316}\\ \hline

Retain Backbone   & AUPR & F1 & \multicolumn{1}{l|}{Kappa} & AUPR & F1 & \multicolumn{1}{l|}{Kappa} & AUPR & F1 & \multicolumn{1}{l|}{Kappa} & AUPR     & F1     & Kappa     \\ \hline
Orginal           &0.6433&0.6174& \multicolumn{1}{l|}{0.4130}      & 0.6366&0.5595& \multicolumn{1}{l|}{0.3235}      &0.4892&0.4588& \multicolumn{1}{l|}{0.1969}      &0.5774&0.4968&0.2759\\
LSTM+MLP          &0.6476&0.6279& \multicolumn{1}{l|}{0.4158}      & 0.6233&0.5757& \multicolumn{1}{l|}{0.3443}      & 0.5065&0.4581& \multicolumn{1}{l|}{0.2033}      &0.5435&0.5210&0.2878\\
LSTM+medGAN       &0.6424&0.6285& \multicolumn{1}{l|}{0.4028}      &0.6403&0.6004& \multicolumn{1}{l|}{0.3653}      &0.5022&0.5223& \multicolumn{1}{l|}{0.2123}      & 0.5577&0.5113&0.2471\\
LSTM+TabDDPM      &0.6465&0.6152& \multicolumn{1}{l|}{0.4067}      &      &    & \multicolumn{1}{l|}{}      &      &    & \multicolumn{1}{l|}{}      &          &        &           \\
EVA               &0.6527&0.6240& \multicolumn{1}{l|}{0.4208}      &      &    & \multicolumn{1}{l|}{}      &      &    & \multicolumn{1}{l|}{}      &          &        &           \\
synTEG            &0.6319&0.6285& \multicolumn{1}{l|}{0.4224}      &0.6496&0.6036& \multicolumn{1}{l|}{0.3783}      &0.4947&0.5074& \multicolumn{1}{l|}{0.2318}      &0.5640&0.5203&0.2923\\
PromptEHR         &0.6582&0.6251& \multicolumn{1}{l|}{0.4211}      &      &    & \multicolumn{1}{l|}{}      &      &    & \multicolumn{1}{l|}{}      &          &        &           \\
TWIN              &0.6540&0.6382& \multicolumn{1}{l|}{0.4187}      & 0.6336&0.5985 & \multicolumn{1}{l|}{0.3840}      &0.5066&0.4816& \multicolumn{1}{l|}{0.2370}      &0.5352&0.5104&0.2860 \\ \hline
Ours              &\textbf{0.6603}&\textbf{0.6397}& \multicolumn{1}{l|}{\textbf{0.4382}}      &\textbf{0.6599}&\textbf{0.6174}& \multicolumn{1}{l|}{\textbf{0.4051}}      &\textbf{0.5105}&\textbf{0.5439}& \multicolumn{1}{l|}{\textbf{0.2631}}      & \textbf{0.5966}&\textbf{0.5307}&\textbf{0.2974}
\end{tabular}
}
\label{heathRisk}
\end{table*}


\begin{table*}[]
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{c|cccc|llll}
Perscent of known patients  & 10 & 20 & 35 & 50 & 10 & 20 & 35 & 50 \\ \hline
\multicolumn{1}{l|}{Metric} & \multicolumn{4}{l|}{PD} & \multicolumn{4}{l}{AD} \\ \hline
LSTM+MLP     & 13.53 & 13.38 & 13.03 & 13.07 & \textbf{7.23} & \textbf{7.30} & \textbf{7.33} & 8.09\\
LSTM+medGAN  & 17.06 & 17.19 & 17.56 & 17.79 & 8.89 & 9.26 & 9.63 & 9.92\\
LSTM+TabDDPM & 13.45 & 13.66 & 13.50 & 13.68 & 8.11 & 8.14 & 8.23 & 8.15\\
EVA          & 13.36 & 13.17 & 12.84 & 13.36 & 7.60 & 7.84 & 8.11 & 8.29\\
synTeg       & 13.21 & 13.02 & 12.71 & 12.76 & 8.81 & 9.05 & 9.30 & 9.91\\
PromptEHR    & 14.44 & 12.86 & 12.90 & 13.31 & 8.60 & 9.35 & 9.90 & 8.22\\
TWIN         & 13.36 & 13.16 & 12.84 & 12.89 & 8.35 & 8.52 & 8.35 & 8.06\\ \hline
Ours         & \textbf{12.60} & \textbf{12.77} & \textbf{12.53} & \textbf{12.25} & 8.03 & 7.70 & 7.76 & \textbf{6.77}
\end{tabular}
}
\label{table:privacy}
\end{table*}


\begin{table*}[]
% \resizebox{0.9\textwidth}{!}
{
\begin{tabular}{l|ll|ll|ll|ll}
\toprule
MIMIC-III & \multicolumn{2}{l|}{Diagnosis} & \multicolumn{2}{l|}{Drug} & \multicolumn{2}{l|}{Lab Item} & \multicolumn{2}{l}{Procedure}\\ \hline
Metric            & lpl          & mpl          & lpl           & mpl           & lpl          & mpl  & lpl          & mpl           \\ \hline
LSTM+MLP         &      325.55     &    352.54    &     553.63      &     551.67      &     168.25     &  166.61  &     290.38      &     286.53      \\
LSTM+medGAN       &    242.30       &    257.48     &    403.02      &     405.75     &    77.10     &  87.12  &      234.81    &     245.28      \\
LSTM+TabDDPM      &     108.79     &      114.18   &     179.22     &    178.70      &    54.69     &   54.44  &    98.03      &   102.72      \\
EVA            &    29.62         &   31.63     &    43.79        &     44.02      &     20.05      &  19.97   &     27.39     &     30.49    \\
synTEG       &   36.87   &       45.61       &    83.38         &     82.66          &   26.80           &     30.34         &  49.33   &        44.00         \\ 
PromptEHR         &   126.23       &    128.05     &     167.48       &    136.04     &     107.22      &   98.52   &      51.18    &  31.13      \\ 
TWIN         &     26.28       &     27.68        &    40.94      &     40.86     &     17.47      &  17.41  &      21.26      &    24.26      \\
\hline
Ours           &   15.97     &    17.95      &   20.53      &    19.15       &    15.11      &  13.99   &    14.53          &    18.89   
\\ 
\bottomrule
\end{tabular}
}
\caption{Experiment Result from MIMIC-III Dataset}
\label{table:fidality_mimic}
\end{table*}

\begin{table*}[]
%\resizebox{0.9\textwidth}{!}
{
\begin{tabular}{l|ll|ll|ll|ll}
\toprule
Breast Cancer Trial & \multicolumn{2}{l|}{Adverse Event} & \multicolumn{2}{l|}{Medication} & \multicolumn{2}{l|}{Lab Category} & \multicolumn{2}{l}{Treatment}\\ \hline
Metric        & lpl & mpl & lpl & mpl & lpl & mpl & lpl & mpl \\ \hline
LSTM+MLP      &8.42 &9.37 &8.82 &8.73 &9.33 &9.22 &7.29 &4.47 \\
LSTM+medGAN   &8.00 &9.42 &9.53 &11.67&10.41&10.08&9.42	&4.83 \\
LSTM+TabDDPM  &9.31 &10.86&11.13&12.95&9.06 &9.03 &3.67 &3.22 \\
EVA           &6.08 &8.30 &5.39 &6.95 &9.07 &9.09 &3.09 &2.89 \\
synTEG        &8.21 &9.70 &8.21 &10.08&9.63 &10.03&9.09 &4.43 \\ 
PromptEHR     &12.37&12.14&19.34&19.80&8.55 &8.66 &5.10 &5.63 \\ 
TWIN          &6.08 &8.52 &5.56 &7.10 &9.09 &9.11 &3.12 &2.92 \\
\hline
Ours          &5.96 &8.02 &4.96 &5.87 &9.01 &9.09 &2.63 &2.41 \\ 
\bottomrule
\end{tabular}
}
\caption{Experiment Result from Breast Cancer Trial Dataset}
\label{table:fidality_breast}
\end{table*}
